Learning to Import through Production Networks

Using administrative data on the universe of inter-firm transactions in Spain, we show that firms learn to import from their domestic suppliers and customers. Our identification strategy exploits the panel structure of the data, the firm-time variation across import origins, and the network structure. We find evidence of both upstream and downstream network effects, even after accounting for sectoral and spatial spillovers. We estimate that an increase of 10 percentage points in the share of suppliers (customers) that are importing from a given region increases the probability of starting importing from that region by 10.7\% (19.2\%). Connections with geographically distant domestic firms provide more useful information to start importing. Larger firms are more responsive to this information but less likely to disseminate it.

==> AdditionalTables/tbl_Network_BasicInfo_NotIncluded.tex <==
%
% Such constructed dataset contains information about on average 10.05 million connections among  firms per year (2010 - 2014) among an average 831525 firms.


% \begin{table}
%     \centering
%     \begin{tabular}{|c|c|c|c|}
%         Year & Number of links &  Number of firms &AverageValueLink\\
%         \hline
%         2010 & 11593279 &  845276 & 74928.26 \\
%         \hline
%         2011 &11200026  &  864986 & 78086.21\\
%         \hline
%         2012 & 10266703 & 848885 & 109908.40 \\
%         \hline
%         2013 & 9896132 & 829947 &  82995.49\\
%         \hline
%         2014 & 9576451  &  768532 & 85430.89\\
%         \hline
%     \end{tabular}
%     \caption{Some information about network. Not to be included in the final version}
%     \label{tab:my_label}
% \end{table}



% \begin{table}
%     \centering
%     \begin{tabular}{|c|c|c|c|}
%         Year & Number of links &  Number of firms &AverageValueLink\\
%         \hline
%         2010 &8736804  &  611996 &  84108.77 \\
%         \hline
%         2011 & 9101097  &  611996 &  86067.78\\
%         \hline
%         2012 & 8758302 & 611996 & 121270.22 \\
%         \hline
%         2013 & 8489903 & 611996 & 88812.95\\
%         \hline
%         2014 &  8273487   &  611996 &  89147.18\\
%         \hline
%     \end{tabular}
%     \caption{Some information about network. Only firms appearing in all years.  Not to be included in the final version}
%     \label{tab:my_label}
%\end{table}


% There are  firms that appear in the network in each year 2010--2014. 
